Information Set Emulation: Causal Certificates for AI Derived EHR Features

AI and large language models can recover clinically meaningful features from electronic health records (EHRs), but predictive usefulness does not establish admissibility for causal inference. We introduce information set emulation: an AI typed lift attaches source evidence, clinical and recording times, decision-time availability, representation version, proposed causal roles, and unresolved ambiguity to extracted features under a locked target trial. Causal certificates record auditable evidence for those roles. Features with unresolved downstream roles are routed to compatible reporting or separate analyses. Typed evidence defines an observational fiber of causal worlds consistent with the observed law. The locked scalar estimand maps this fiber to a compatible image whose squared Chebyshev radius equals the residual minimax mean squared error when the image is nonempty and compact. This classical identity provides a target-specific measure of information ambiguity. The contribution is its integration with a joint EHR observation map and an auditable certificate architecture. Under explicit exchangeability, positivity, and nuisance-consistency conditions, we give identification and cross-fitted augmented inverse probability weighted estimation, distinguishing empirical and population targets. An EHR compression-drift identity separates the roles of frame presence, treatment assignment, and outcome observation. Artificial simulations and a common-law finite-world example illustrate estimation failures and information-radius reduction. Synthetic Phase 0 notes demonstrate audit diagnostics; a separate role-specific analysis spread illustrates routing and is not an exact fiber radius. All experiments are synthetic. The framework specifies when reconstructed information can support a point claim and when compatible reporting is required.

==> tables/TableAdditionalStress.tex <==
\begin{tabular}{llrrr}
\toprule
Failure mode & Setting & Bias & RMSE & Coverage \\
\midrule
AI extraction error & low extraction error & 0.005 & 0.103 & 0.980 \\
AI extraction error & moderate extraction error & 0.266 & 0.293 & 0.435 \\
AI extraction error & high extraction error & 0.497 & 0.514 & 0.050 \\
Post index partial leakage & no leakage lambda 0 & 0.011 & 0.114 & 0.935 \\
Post index partial leakage & partial leakage lambda 0.25 & -0.308 & 0.323 & 0.115 \\
Post index partial leakage & partial leakage lambda 0.50 & -0.423 & 0.433 & 0.005 \\
Certificate role misclassification & misclassification 0 percent & 0.024 & 0.112 & 0.970 \\
Certificate role misclassification & misclassification 10 percent & -0.169 & 0.202 & 0.625 \\
Certificate role misclassification & misclassification 20 percent & -0.305 & 0.319 & 0.105 \\
Availability error & available at time zero & 0.017 & 0.106 & 0.950 \\
Availability error & late availability lambda 0.50 & -0.818 & 0.822 & 0.000 \\
Availability error & late availability lambda 1.00 & -1.103 & 1.106 & 0.000 \\
Positivity stress & ordinary overlap & 0.011 & 0.116 & 0.920 \\
Positivity stress & strong positivity stress & 0.023 & 0.140 & 0.940 \\
\bottomrule
\end{tabular}

==> tables/TableMainSimulation.tex <==
\begin{tabular}{lrrrrrr}
\toprule
Method & True & Estimate & Bias & RMSE & Mean SE & Coverage \\
\midrule
Structured EHR estimator & 0.644 & 1.391 & 0.747 & 0.761 & 0.140 & 0.001 \\
Naive AI estimator & 0.644 & 0.140 & -0.503 & 0.513 & 0.095 & 0.000 \\
ISE causal estimator & 0.644 & 0.657 & 0.013 & 0.115 & 0.111 & 0.938 \\
Design erasure estimator & 0.644 & 1.026 & 0.383 & 0.404 & 0.126 & 0.146 \\
Post index leakage estimator & 0.644 & 0.164 & -0.479 & 0.491 & 0.100 & 0.000 \\
Oracle prospective estimator & 0.644 & 0.645 & 0.002 & 0.114 & 0.110 & 0.941 \\
\bottomrule
\end{tabular}
